Supernova remnants: the X-ray perspective

Supernova remnants are beautiful astronomical objects that are also of high scientific interest, because they provide insights into supernova explosion mechanisms, and because they are the likely sources of Galactic cosmic rays. X-ray observations are an important means to study these objects.And in particular the advances made in X-ray imaging spectroscopy over the last two decades has greatly increased our knowledge about supernova remnants. It has made it possible to map the products of fresh nucleosynthesis, and resulted in the identification of regions near shock fronts that emit X-ray synchrotron radiation. In this text all the relevant aspects of X-ray emission from supernova remnants are reviewed and put into the context of supernova explosion properties and the physics and evolution of supernova remnants. The first half of this review has a more tutorial style and discusses the basics of supernova remnant physics and thermal and non-thermal X-ray emission. The second half offers a review of the recent advances.The topics addressed there are core collapse and thermonuclear supernova remnants, SN 1987A, mature supernova remnants, mixed-morphology remnants, including a discussion of the recent finding of overionization in some of them, and finally X-ray synchrotron radiation and its consequences for particle acceleration and magnetic fields.

==> jvink_aarv_tab_mixed.tex <==
\begin{table*}
\begin{center}
\caption{Mixed morphology SNRs.\label{tab:mixed}}
{\small
\begin{tabular}{lllllllllll}\hline\hline\noalign{\smallskip}

SNR	&	Name	&	Size	&	$F_{\rm R}$	&	$\alpha_{\rm R}$	&	Dist	&Enh. 	&	RRC	&	GeV 	&	TeV 	& OH 		\\
	&		&		&		&		&		&	metals & 	&		&		&		Maser	\\
	&		&	arcmin	&	Jy	&		&kpc		&		&		&		&		&			\\
\noalign{\smallskip}\hline
\noalign{\smallskip}
G0.0+0.0	&	Sgr A East 	&	$3.5\times 2.5$	&	100?	&	0.8?	&	8	&	X	&		&	?	&	?	&	X (v)	\\
G6.4â0.1	&	W28	&	48	&	310	&	0.3	&	1.9	&		&		&	X (c)	&	X (g)   &	X (n)	\\
G31.9+0.0	&	3C391	&	$7\times 5$	&	24	&	0.49	&	8.5	&		&		&	X (k)  &		&	X (n)	\\
G33.6+0.1	&	Kes 79	&	10	&	22	&	0.5	&	7.8	&		&		&		&		&		\\
G34.7â0.4	&	W44	&	$35\times 27$	&	230	&	0.37	&		&	X	&		&	X (e)	&		&	X (n)	\\
G41.1â0.3	&	3C397	&	$4.5\times2.5$	&	22	&	0.48	&	7.5	&	X	&		&		&		&		\\
G43.3â0.2	&	W49B	&	4	&	38	&	0.48	&	10	&	X	&	X (s)	&	X (d)	&	X (j)	&		\\
G49.2â0.7	&	W51C	&	30	&	160	&	0.3	&	6	&		&		&	X (a)	&	X (y)	
&	X (o)	\\
G53.6â2.2	&	3C400.2	&	$33\times 28$	&	8	&	0.75	&	2.8	&		&		&		&		&		\\
G65.3+5.7	&	G65.3+5.7	&	$310\times 240$	&	52?	&	0.6?	&	0.8	&		&		&		&		&		\\
G82.2+5.0	&	W63	&	$95\times 65$	&	120	&	0.35	&		&	X	&		&		&		&		\\
G89.0+4.7	&	HB21	&	$120\times 90$	&	220	&	0.48	&	0.8	&	X	&		&		&		&		\\
G93.7â0.2	&	CTB 104A	&	80	&	65	&	0.65	&	1.5	&		&		&		&		&		\\
G116.9+0.2	&	CTB1	&	34	&	8	&	0.61	&		&	X	&		&		&		&		\\
G132.7+1.3	&	HB3	&	80	&	45	&	0.6	&	2.2	&	X	&		&	X (b)	&		&		\\
G156.2+5.7	&	G156.2+5.7	&	110	&	5	&	0.5	&		&	X	&		&		&		&		\\
G160.9+2.6	&	HB9	&	$140 \times 120$	&	110	&	0.64	&	$<4$	&		&		&		&		&		\\
G166.0+4.3	&	VRO 42.05.01	&	$55\times 35$	&	7	&	0.37	&	4.5	& X (h)	&		&		&		&		\\
G189.1+3.0	&	IC 443	&	45	&	160	&	0.36	&	1	&	X (h)	&	X (x)	&	X (f)	&	X (h)	&	X (m)	\\
G272.2-3.2	&	G272.2-3.2	&	15?	&	0.4	&	0.6	&	2?	&	X (s)	&		&		&		&		\\
G290.1-0.8	&	MSH 11-61A	&	19x14	&	42	&	0.4	&	7	&	X			&	X (b)	&		&		\\
G327.4+0.4	&	Kes 27	&	21	&	30	&	0.5	&	5	&	X (k)	&		&		&		&		\\
G327.1-1.1	&	G327.1-1.1	&	7	&	18	&	0.36	&		&		&		&		&		&		\\
G357.1-0.1	&	Tornado	&	$8\times 3$	&	37	&	0.4	&	$>8$	&		&		&		&		&		\\
G359.1-0.5	&	G359.1-0.5	&	24	&	14	&	0.4	&		& X		& X (r)		&		&		&	X (q)	\\
\noalign{\smallskip}\hline
\end{tabular}
}
\end{center}
\scriptsize{
This list is based on the list by  \citet{lazendic06b}.
Sizes, distances, and radio properties (radio flux $F_{\rm R}$, and spectral index $\alpha_{\rm R}$)
were obtained from
Green D. A., 2009, ``A Catalogue of Galactic Supernova Remnants 
(2009 March version)'', Astrophysics Group, Cavendish Laboratory, Cambridge, United Kingdom (available at \url{http://www.mrao.cam.ac.uk/surveys/snrs/}.
The column names indicate: Enh. metals, the presence of plasma with overbaundances \citep[][unless indicated otherwise]{lazendic06b};
RRC, the presence of radiative recombination-line continua; GeV, the detection in the GeV band (\fermi); TeV the detection of associated sources
in the TeV band with Cherenkov telescopes; OH Maser, the detection of associated OH masers.
The letters in parentheses refer to the following references:\\
a) \citet{abdo09}; 
b) \citet{abdo10e}; 
c) \citet{abdo10c}; 
d) \citet{abdo10d}; 
e) \citet{abdo10b};
f) \citet{abdo10f}; 
g) \citet{aharonian08a}; 
h) \citet{albert07b};
i) \citet{bocchino09};
j) \citet{brun11};
k) \citet{castro10}; 
l) \citet{chen08}
m) \citet{claussen97}; 
n) \citet{frail96} ; 
o) \citet{green97}
p) \citet{koralesky98b}; 
q) \citet{lazendic02};
r) \citet{ohnishi11};
s) \citet{ozawa09};
t) \citet{park09};
u) \citet{yusef-zadeh95};
v) \citet{yusef-zadeh96};
w) \citet{yusef-zadeh99};
x) \citet{yamaguchi09};
y) \citet{feinstein09}; \citet{krause11}.
}
\end{table*}

